Energy-Efficient Internet of Things Monitoring with Content-Based Wake-Up Radio

The use of Wake-Up Radio (WUR) in Internet of Things (IoT) networks can significantly improve their energy efficiency: battery-powered sensors can remain in a low-power (sleep) mode while listening for wake-up messages using their WUR and reactivate only when polled. However, polling-based WUR may still lead to wasted energy if values sensed by the polled sensors provide no new information to the receiver, or in general have a low Value of Information (VoI). In this paper, we design a content-based WUR that tracks the process observed by the sensors and only wakes up the sensor if its estimated update's VoI is higher than a threshold communicated through the poll. If the sensor does not reply to the polling request, the Gateway (GW) can make a Bayesian update, knowing that either the sensor value substantially confirms its current estimate or the transmission failed due to the wireless channel. We analyze the trade-off between the tracking error and the battery lifetime of the sensors, showing that content-based WUR can provide fine-grained control of this trade-off and significantly increase the battery lifetime of the node with a minimal Mean Squared Error (MSE) increase.

==> extra.tex <==

We can find an approximate solution by using the Taylor series of the Gaussian \gls{cdf} function $\Phi(x)$:
\begin{equation}\label{eq:taylor}
    \Phi(x) \simeq \frac{1}{2}+\frac{1}{\sqrt{2\pi}}\sum_{\ell=0}^{\infty}\frac{(-1)^{\ell} x^{2\ell+1}}{\ell!(2\ell+1)}.
\end{equation}
The tenth-order Taylor approximation provides a good enough approximation for $-1\leq x\leq 1$:
\begin{equation}
    \erf\left(\frac{x}{\sqrt{2}}\right) = \sqrt{\frac{2}{\pi}}\Bigg[x-\frac{x^3}{6}+\frac{x^5}{40}-\frac{x^7}{336}+\frac{x^9}{3456}\Bigg].
\end{equation}
Hence, \eqref{eq:variance_integral} can be rewritten as:
\begin{equation}\label{eq:variance_full}
\begin{aligned}
    P_{m,n}(k|\xi)=&\frac{2P_{m,n}}{P_{n,n}}\int_{1}^{\infty} p(z_n|\xi)z_n^2\ dz_n\\
    &+\frac{P_{m,n}}{P_{n,n}}\int_{-1}^{1} p(z_n|\xi)z_n^2\ dz_n.
\end{aligned}
\end{equation}
As the first integral term goes from $1$ to $\infty$, we can find a simple upper bound to the Gaussian \glspl{cdf}:
\begin{equation}
    \Phi\left(\!\frac{-z_n-\theta}{\sqrt{P_{n,n}}}\!\right)+\Phi\left(\!\frac{\theta-z_n}{\sqrt{P_{n,n}}}\!\right) \leq \Phi\left(\!\frac{-1-\theta}{\sqrt{P_{n,n}}}\!\right)+\Phi\left(\!\frac{\theta-1}{\sqrt{P_{n,n}}}\!\right).
\end{equation}
Hence,~\eqref{eq:variance_full} is bounded by:
\begin{equation}\label{eq:variance_bound}
\begin{aligned}
    P_{m,n}(k|\xi)\leq&\frac{2P_{m,n}}{p_n(\xi)}\left(\Phi\left(\!\frac{-1-\theta}{\sqrt{P_{n,n}}}\!\right)+\Phi\left(\!\frac{\theta-1}{\sqrt{P_{n,n}}}\!\right)\right)\\
    &+\frac{P_{m,n}}{P_{n,n}}\int_{-1}^{1} p(z_n|\xi)z_n^2\ dz_n.
\end{aligned}
\end{equation}
Using the Taylor series approximation from~\eqref{eq:taylor} to solve the second integral, we get:
\begin{equation}\label{eq:variance_approx}
\begin{aligned}
    P_{m,n}(k|\xi)\lesssim&\frac{2P_{m,n}}{p_n(\xi)}\left(\Phi\left(\!\frac{-1-\theta}{\sqrt{P_{n,n}}}\!\right)+\Phi\left(\!\frac{\theta-1}{\sqrt{P_{n,n}}}\!\right)\right)\\
    &\Bigg[\mathbf{\Phi}\Big(\frac{\mathbf{1}+\epsilon}{\sigma_{\mathbf{\hat{x}}_{pri}}}\Big)-\mathbf{\Phi}\Big(\frac{\mathbf{1}-\epsilon}{\sigma_{\mathbf{\hat{x}}_{pri}}}\Big) + \sum_{i=1}^{9}(i~\mathbf{mod}~2)~\epsilon^i\Bigg]
\end{aligned}
\end{equation}
The computation can be repeated for all the elements of the $n$-th column of $\mathbf{P}(k)$, completing the update.
%To compute the variance of the truncated gaussian, we consider the bayes theorem,
%In that case, as we know that the value resides between the two truncation limits, we define the measurement values required to update the filter parameters as the expectation of the truncated gaussian of the \textit{a priori} estimates which
Note that, this computations are only true for one dimensional error estimates. So we assume that each dimension in the $P$-dimensional process resembles independent events happening in the area and hence can be estimated independently by the kalman filter. Hence, we can consider the truncation over the entire estimate vector to be independent for the system. Additionally, there is also a challenge in choosing the $\epsilon$ that would allow to maximise the \gls{voi} obtained.
\subsection{Scheduling Strategy}

